RoboPARA: Dual-Arm Robot Planning with Parallel Allocation and Recomposition Across Tasks

Dual-arm robots play a crucial role in improving efficiency and flexibility in complex multitasking scenarios. While existing methods have achieved promising results in task planning, they often fail to fully optimize task parallelism, limiting the potential of dual-arm collaboration. To address this issue, we propose RoboPARA, a novel large language model (LLM)-driven framework for dual-arm task parallelism planning. RoboPARA employs a two-stage process: (1) Dependency Graph-based Planning Candidates Generation, which constructs directed acyclic graphs (DAGs) to model task dependencies and eliminate redundancy, and (2) Graph Re-Traversal-based Dual-Arm Parallel Planning, which optimizes DAG traversal to maximize parallelism while maintaining task coherence. In addition, we introduce the Cross-Scenario Dual-Arm Parallel Task dataset (X-DAPT dataset), the first dataset specifically designed to evaluate dual-arm task parallelism across diverse scenarios and difficulty levels. Extensive experiments demonstrate that RoboPARA significantly outperforms existing planning methods, achieving higher efficiency and reliability, particularly in complex task combinations. Our code is publicly available at https://github.com/AiDuanshiying/RoboPARA.

==> sections/method.tex <==
\section{Methodology}
\label{Method}

\subsection{Problem Formulation}

We formally define a new task, the \textbf{Dual-Arm Cooperative Scheduling Problem}, as follows:
We consider the problem of scheduling a set of \( m \) tasks, where each task \( i \) consists of \( n_i \) sequential operations to be performed on two cooperative robotic arms, denoted as \( L \) and \( R \).
Each operation \( o_{ij} \) (the \( j \)-th operation of task \( i \)) is either a {single-arm operation}, which can be executed by either \( L \) or \( R \) individually, or a {dual-arm operation}, which requires synchronized execution by both arms.
The objective is to minimize the \textbf{makespan} \( C_{\max} \), defined as the total time required to complete all operations across all tasks, while respecting the task dependencies and resource constraints.
The makespan is expressed as:
\[
C_{\max} = \max_{i \in \{1, \dots, m\}} \Bigg( \max_{j \in \{1, \dots, n_i\}} \big( s_{ij} + p_{ij} \big) \Bigg),
\]
where \( s_{ij} \) denotes the start timestamp of operation \( o_{ij} \), and \( p_{ij} \) is its processing time.
This formulation ensures that the completion timestamp of the last operation across all tasks is minimized, balancing parallelism and synchronization between the two robotic arms.
The problem is subject to the following three constraints:
\begin{itemize}
    \item \emph{Grasping Constraint:} At any time, each manipulator (arm \( L \) or \( R \)) is restricted to interacting with at most one object. Once an arm begins operating on an object, it must either complete all associated operations or explicitly release the object before interacting with another.
    \item \emph{Dual-Arm Synchronization Constraint:} Dual-arm operations require both arms to begin execution simultaneously and remain continuously engaged for the full duration of the task.%Dual-arm operations must be executed by both arms simultaneously, with synchronized start times, and both arms remain engaged throughout the operation's duration.
    \item \emph{Operation Batching Constraint:} To reduce setup and teardown overhead, identical operations occurring in multiple tasks (such as using the same tool on different objects) may be grouped and executed as a batch.%Identical operations across multiple tasks (e.g., processing different objects using the same tool) can be batched together to amortize setup and teardown costs.
\end{itemize}

The problem is to minimizes \( C_{\max} \) while ensuring the feasibility of execution.
%By solving this problem, we aim to design an optimized task schedule that minimizes \( C_{\max} \) while ensuring the feasibility of execution under these constraints.


\input{figs/RoboPARA_framework}


\subsection{Overview}

As shown in Fig.~\ref{pipline_1.0}, our hardware setup consists of two collaborative robotic arms, and the proposed planning framework, which we term RoboPARA, is designed to efficiently coordinate these arms for executing complex tasks.
RoboPARA takes natural language user instruction as input, specifying key requirements and scenario details (e.g., ``Please make me carrot slices and a cream bread'').
Leveraging the robots' observations and long-term memory (e.g., task execution history and environmental knowledge), RoboPARA extracts the necessary contextual information and task steps to guide execution.
To address the newly defined Dual-Arm Cooperative Scheduling Problem, RoboPARA ensures both task correctness and optimal utilization of the robotic arms through a two-stage architecture: Dependency Graph-based Planning Candidate Generation and Graph Re-Traversal-based Dual-Arm Parallel Planning (Alg.~\ref{main_alg}).
The first stage focuses on generating multiple planning candidates, while the second stage optimizes these candidates and selects the optimal one.
The output of RoboPARA is a complete, time-synchronized execution plan for the dual-arm system, detailing the specific meta actions, their expected execution time based on empirical estimates, and the assignment of each action to one or both arms.
In the following sections, we provide a detailed explanation of these two stages, highlighting the key components and innovations of our approach.

\subsection{LLM-Driven Dependency Graph for Planning Candidates Generation}
The first stage of our framework focuses on generating a DAG to represent the task structure and serve as the basis for exploring different execution possibilities. When a user provides a natural language instruction, the system retrieves relevant task records from the knowledge base using RAG.
These records include task names and detailed steps, derived by comparing the input with prior execution records stored in both the robots' short-term observations (e.g., images, object states) and long-term memory (e.g., task history and environmental knowledge).

Once the task steps are retrieved, the system integrates additional contextual information, such as environmental states, dependency rules (including node dependency restrictions, action type classifications, and action parallelism prompts), output formats, and example inputs and outputs into a prompt.
The relevant prompt is provided in Appendix Sec.~\ref{full_prompt}.
This prompt is then input to a LLM to generate the initial DAG.
The nodes in the DAG are categorized into four types: \textit{Pick}, \textit{Use}, \textit{Place}, and \textit{Open/Close}.
Dependency rules are applied to ensure logical consistency and minimize potential deadlocks.
For instance, a \textit{Use} node must depend on the corresponding \textit{Pick} node of the same tool, a \textit{Place} node must depend on its preceding \textit{Use} node, and tool usage operations must consider the last \textit{Use} node to maintain sequential correctness.

Since the initial DAG may contain errors in dependency relationships, the system also performs error detection by validating the graph against predefined rules (ref.~Alg.~\ref{very_DAG}).
The system focuses on three types of errors: (1) when the \textit{Use} or \textit{Place} node of an object depends on the \textit{Place} node of another object, (2) when a \textit{Place} node in a \textit{Pick-Use-Place} sequence directly depends on its \textit{Pick} node instead of the preceding \textit{Use} node, and (3) when a node incorrectly depends on the \textit{Use} node of another object.
After identifying these errors and their corresponding node IDs, the system integrates the error types, node IDs, the original DAG, dependency relationship rules, and output formats into a new prompt.
The relevant prompt is detailed in Appendix Sec.~\ref{full_prompt}.
This updated prompt is sent back to the LLM for correction.
%If the corrected DAG still contains errors, at most one additional correction attempt is made.
Once a finalized DAG is generated, it is passed to the next stage for traversal-based selection of the optimal plan.

\subsection{Graph Re-Traverse for Parallel Optimal Dual-Arm Planning}
In this stage, we use the validated DAG from the previous step to generate an optimal task execution plan.
This is achieved through two main steps: dynamically scheduling tasks and resolving potential deadlocks, as illustrated in Fig.~\ref{pipline_1.0}.

First, the DAG is converted into structured node objects, where each node contains task type (e.g., pick, place, cut), resource requirements (single-arm or dual-arm), execution time, and dependency relationships (predecess and successor actions).
These dependencies define the execution order of actions.
Nodes without any prerequisites are added to the scheduling queue immediately.
These actions are then allocated dynamically based on their type and the state of the robotic arms.
For single-arm actions, the system assigns the action to the arm that has been idle longer; in case of a tie, the left arm is prioritized.
For dual-arm tasks, such as cutting or moving large objects, both arms are synchronized to execute the task simultaneously, ensuring their execution times overlap completely.
If an arm becomes locked to an object chain after a pick task (e.g., holding a knife), all subsequent tasks related to that object must be executed by the same arm to avoid conflicts.
The specific details of the arm selection algorithm can be found in the Appendix~Alg.~\ref{alg:choose_arm}.

If the system detects that a dual-arm action cannot proceed due to conflicting pick operations (e.g., each arm holding different objects), it triggers deadlock handling.
To resolve the conflict, the system rolls back the pick task executed later.
For instance, if the right arm's pick task is the cause of the conflict, it is removed along with its dependent tasks, freeing the right arm's object lock.
These removed tasks are then re-added to the scheduling event queue, allowing the earlier pick task to proceed.
Subsequently, the dual-arm task (e.g., cutting) is reassigned to the arm holding the required object chain (e.g., the left arm), ensuring both arms are synchronized for execution.
This rollback mechanism effectively breaks the deadlock and restores the continuity of the task sequence.
The pseudo code for the scheduling and deadlock handling logic is shown in the Appendix~Alg. ~\ref{scheduler_alg}.

By combining a robust scheduling mechanism with proactive deadlock resolution, this stage ensures efficient dual-arm collaboration while adhering to task dependencies.
It minimizes idle time and selects the optimal task execution plan to achieve the desired outcomes. 

% \subsection{Problem Formulation}
% We formalize the \textbf{Dual-Arm Cooperative Scheduling Problem} as a temporally and structurally constrained optimization problem over a set of task packages to be completed by two robotic arms. Let \(\mathcal{P} = \{P_1, P_2, \dots, P_m\}\) denote the collection of packages, where each \(P_i\) is composed of a sequence of atomic operations.

% All operations across all packages are aggregated into a global directed acyclic graph (DAG) \(\mathcal{G} = (\mathcal{V}, \mathcal{E})\), where each node \(v \in \mathcal{V}\) corresponds to an atomic operation, represented as a tuple \((\texttt{name}_v, \texttt{type}_v, \delta_v, t_v)\). This tuple specifies the action label, semantic type, required number of arms \(\delta_v \in \{1, 2\}\), and execution duration \(t_v \in \mathbb{R}^+\). Each directed edge \((v_i \rightarrow v_j) \in \mathcal{E}\) encodes a precedence constraint, indicating that operation \(v_j\) must not begin before \(v_i\) finishes.

% Let \(\mathcal{A} = \{L, R\}\) be the set of available robotic arms. We define an arm assignment function:
% \begin{equation}
%     \mu: \mathcal{V} \rightarrow \mathcal{P}(\mathcal{A}), \quad \text{with } |\mu(v)| = \delta_v,
% \end{equation}
% which allocates each operation to its responsible arm(s), subject to exclusivity and synchronization semantics.

% We further define a scheduling function \(\sigma: \mathcal{V} \rightarrow \mathbb{R}^+\), assigning each node a non-negative start time. The pair \((\sigma, \mu)\) must satisfy all task dependencies, arm availability constraints, and consistency requirements throughout execution.

% The effectiveness of any dual-arm execution plan is measured by its \textbf{makespan}—the total time required to complete all scheduled operations. Formally, the makespan is defined as the maximum completion time over all operations in the graph:
% \begin{equation}
%     C_{\max} := \max_{v \in \mathcal{V}} \left( \sigma(v) + t_v \right).
% \end{equation}

% Our objective is to find a valid schedule and arm assignment that jointly minimize this makespan:
% \begin{equation}
%     \min_{\sigma, \mu} \; C_{\max}, \quad \text{subject to } (\sigma, \mu) \in \mathcal{F}(\mathcal{G}, \mathcal{S}),
% \end{equation}
% where \(\mathcal{S}\) denotes the current environment state (e.g., object locations, initial arm occupancy), and \(\mathcal{F}(\mathcal{G}, \mathcal{S})\) represents the feasible set of schedule-allocation pairs adhering to all structural, temporal, and contextual constraints.

% \subsection{Overall Framework}
% RoboPARA tackles the newly defined \textbf{Dual-Arm Cooperative Scheduling Problem} through a two-stage architecture: \textbf{Dependency Graph-based Planning Candidate Generation} and \textbf{Graph Re-Traversal-based Dual-Arm Parallel Planning}. The overall framework is illustrated in \textbf{Fig.~\ref{pipline_1.0}}.
% The first stage focuses on generating multiple planning candidates, while the second stage performs efficient parallel scheduling, selecting the optimal execution plan.
% The final output is a complete, time-synchronized execution plan detailing atomic operations, durations, and arm assignments, ensuring task correctness and efficient arm utilization.
% The following sections elaborate on each stage of RoboPARA, detailing the core algorithmic components and innovations underlying our design.

% \subsection{LLM-Driven Dependency Graph for Planning Candidates Generation}

% The first stage of RoboPARA constructs the task-level DAG \(\mathcal{G} = (\mathcal{V}, \mathcal{E})\), serving as the structural foundation for dual-arm scheduling. Given a user-issued natural language instruction, RoboPARA employs the RAG  approach to fetch relevant task knowledge from a hybrid memory system. This memory integrates both short-term sensor observations (e.g., object states) and long-term execution history (e.g., package knowledge base).

% The retrieved task steps are then augmented with additional contextual information—such as environmental constraints, dependency rules, parallelism guidelines, and structured formatting examples—to form a full prompt (Appendix Sec.~\ref{full_prompt}). This prompt is submitted to a LLM, which produces an initial instance of \(\mathcal{G}\), where each node \(v \in \mathcal{V}\) is categorized into operation types such as \texttt{pick}, \texttt{use}, \texttt{place}, \texttt{open}/\texttt{close} and \texttt{complete}. The LLM-generated dependency edges \(\mathcal{E}\) are required to reflect logical precedence constraints—for example, a \texttt{use} action must follow a corresponding \texttt{pick}  of the same tool, and a \texttt{place} must not precede the associated \texttt{use}. Additionally, tool-related action sequences must maintain intra-object dependency consistency. The \texttt{complete} node serves as the unique sink of \(\mathcal{G}\), aggregating all terminal dependencies to represent the logical end of the task sequence.

% Since the initial \(\mathcal{G}\) may contain errors in dependency relationships, we apply a structural validation routine (Alg.~\ref{very_DAG}) to detect and localize errors. Three key categories of invalid dependencies are identified:  
% (1) an operation (\texttt{use} or \texttt{place}) incorrectly depending on another object's \texttt{place};  
% (2) a \texttt{place} node in a \texttt{pick-use-place} sequence directly depends on its \texttt{pick} node instead of the preceding \texttt{use} node;  
% (3) any node depending on the \texttt{use} node of an unrelated other object.

% Once errors are identified, their associated nodes and dependency relationship rules are integrated into a new prompt for iterative correction (Appendix Sec.~\ref{full_prompt}). This updated prompt is then re-submitted to the LLM to regenerate a structurally valid \(\mathcal{G}\). Upon successful validation, the resulting task graph \(\mathcal{G}\) is passed to the next stage for scheduling and traversal-based execution planning.


% \subsection{Graph Re-Traverse for Parallel Optimal Dual-Arm Planning}

% Given a validated task graph \(\mathcal{G} = (\mathcal{V}, \mathcal{E})\) from the previous stage, the second stage of RoboPARA constructs a feasible and efficient dual-arm execution plan. This planning process builds a valid pair \((\sigma, \mu)\), assigning each node \(v \in \mathcal{V}\) a start time \(\sigma(v)\) and a responsible arm set \(\mu(v) \subseteq \mathcal{A}\), such that the overall makespan \(C_{\max}\) is minimized while respecting all structural and physical constraints.

% \textbf{Scheduling Framework.} We maintain a dynamic scheduling queue \(\mathcal{Q}\), initialized with all nodes \(v\) that satisfy:
% \begin{equation}
%     \texttt{Ready}(v) := \{v \in \mathcal{V} \mid \text{ all predecessors } u \in \text{pred}(v) \text{ are scheduled}\}
% \end{equation}
% Each node in \(\mathcal{Q}\) is evaluated and assigned based on arm availability, task type (\(\delta_v = 1\) or \(2\)), and object-holding consistency. Single-arm tasks are allocated to the currently idle arm; in case of a tie, the left arm is prioritized. Dual-arm tasks are assigned only if both arms are simultaneously available and not object-locked.

% \textbf{Formal Constraints.} To ensure correctness and feasibility, the plan \((\sigma, \mu)\) must satisfy the following four categories of constraints:
% \begin{enumerate}
%     \item \textbf{Task Dependency.} 
%     Each task \(v \in \mathcal{V}\) can only be scheduled after the completion of all its predecessors. Formally:
%     \begin{equation}
%         \sigma(v) \geq \max_{u \in \text{pred}(v)} \left( \sigma(u) + t_u \right),
%     \end{equation}
%     where \(\text{pred}(v) := \{u \in \mathcal{V} \mid (u \rightarrow v) \in \mathcal{E} \}\) denotes the set of immediate predecessors of \(v\).
    
%     \item \textbf{Unlocked Arm Availability.}
%     Each robotic arm \(a \in \mathcal{A}\) can execute at most one operation at any given time. An operation \(v \in \mathcal{V}\) is schedulable only if all arms in \(\mu(v)\) are free throughout its entire execution interval, formally:
%     \begin{equation}
%         \forall v, v' \in \mathcal{V},\; v \neq v',\; \mu(v) \cap \mu(v') \neq \emptyset \;\Rightarrow\;
%         [\sigma(v), \sigma(v) + t_v) \cap [\sigma(v'), \sigma(v') + t_{v'}) = \emptyset.
%     \end{equation}

%     \item \textbf{Arm Lock Compatibility.}
%     Each \texttt{pick-use-place} sequence involving the same object must be executed by the same arm(s):
%     \begin{equation}
%         \forall (v_{\texttt{pick}}, v_{\texttt{use}}, v_{\texttt{place}}) \in \mathbb{S},\quad \mu(v_{\texttt{pick}}) = \mu(v_{\texttt{use}}) = \mu(v_{\texttt{place}}),
%     \end{equation}
%     where \(\mathbb{S}\) denotes the set of all pick-use-place triples extracted from \(\mathcal{G}\).

%     \item \textbf{Deadlock Prevention.}
%     If a dual-arm task \(v_d\) becomes ready but cannot be executed because each arm \(a \in \mu(v_d) = \{L, R\}\) is currently locked to a different object, a potential deadlock is detected. To resolve it, we identify the \texttt{pick} action \(v_{\text{late}}\) that was executed later among the two conflicting chains and rolls it back along with its dependent subtree:
%     \begin{equation}
%         \texttt{Rollback}(v_{\text{late}}) := \text{Descendants}(v_{\text{late}}) \cup \{v_{\text{late}}\}.
%     \end{equation}
%     These removed operations are then re-inserted into the scheduling queue \(\mathcal{Q}\), freeing the corresponding arm and allowing the earlier pick chain to proceed. The dual-arm task \(v_d\) is subsequently rescheduled once both arms are synchronized and the required object chain is held by one side.
% \end{enumerate}

% \textbf{Execution Procedure.} Scheduling proceeds iteratively: at each step, the system selects a feasible task pair (e.g., one or two nodes from \(\mathcal{Q}\)) and assigns them to arms based on priority and constraint satisfaction. When a dual-arm task is scheduled, both arms are synchronized, ensuring \(\sigma_L(v) = \sigma_R(v) = \sigma(v)\) where \(v\) is a node with \(\delta_v = 2\). Object lock status is updated after each pick action, and all subsequent tasks referencing the same object are bound to the same arm via Constraint 3. 
% If no feasible pair can be scheduled due to conflict or lack of readiness, the system invokes rollback per Constraint 4, prioritizing preservation of earlier actions.

% The full scheduling and rollback algorithm is detailed in Appendix~Alg.~\ref{scheduler_alg}. This mechanism ensures that task dependencies are respected, resource conflicts are avoided, and execution efficiency is maintained throughout dual-arm parallel coordination.

==> sections/problem.tex <==
% \section{Shortest-Time Planning for Multi-Tasks Executed in Parallel by Dual Arms}
% \label{headings}

% \subsection{Task Objective }

% Task Objective: Given a set of multi-tasks and the physical constraints of the dual robotic arms, plan the action sequences of the two arms to minimize the completion time of all tasks, while avoiding action conflicts and deadlocks. The objective function is constructed as follows:

% Let $T$ be the total time to complete all package tasks, $t_{ij}$ denote the time taken by the robot to execute the $j$-th task step of the $i$-th package, $n_i$ be the number of task steps included in the $i$-th package, and $m$ be the total number of packages. Then the objective function can be expressed as:
% \begin{equation}
% T = \min \sum_{i = 1}^{m}\sum_{j = 1}^{n_i}t_{ij}
% \end{equation}
% This objective function aims to reduce the waiting time between tasks and repetitive operations by arranging the task execution sequence reasonably, so as to achieve the goal of minimizing the overall task execution time. For example, when there are the same operations (such as cutting an object) in different packages, these same operations are executed centrally through optimized planning, reducing the number of times of picking up and placing the tool, and thus shortening the total time.

% \subsection{Constraints}
% \subsubsection{Operation Constraints}
% %\textbf{Single-Arm Single-Grasping Constraint: }
% Let the left arm and the right arm of the robot be $L$ and $R$ respectively. For any time instant $k$, a single arm can only grasp one object at the same time. Let $x_{ijk}^L$ and $x_{ijk}^R$ represent whether the left arm and the right arm grasp an object when executing the $j$-th task step of the $i$-th package. If grasping, the value is 1, otherwise it is 0. Then the constraint conditions are:
% \begin{equation}
%     \sum_{j = 1}^{n_i}x_{ijk}^L \leq 1, \sum_{j = 1}^{n_i}x_{ijk}^R \leq 1, \forall i,k
% \end{equation}


% Single-Arm Object-Holding Operation Constraint: When an arm is holding an object, it can only perform operations related to that object or put down that object. Let $o_{ij}$ represent the object involved in the $j$-th task step of the $i$-th package, and $a_{ij}$ represent the operation type of this task step. If an arm is holding an object $o$, then the current operation $a$ must be related to $o$ (for example, when holding a knife, only operations like cutting an object or putting down the knife can be performed). It can be expressed as:

% \begin{equation}
%     x_{ijk}^L = 1 \Rightarrow (a_{ij} \text{ is related to } o_{ij} \text{ or } a_{ij} = \text{put down } o_{ij}), \forall i,j,k
% \end{equation}

% \begin{equation}
%     x_{ijk}^R = 1 \Rightarrow (a_{ij} \text{ is related to } o_{ij} \text{ or } a_{ij} = \text{put down } o_{ij}), \forall i,j,k
% \end{equation}

% %\subsubsection{Dual-Arm Action Constraints}
% Dual-arm actions must be executed by both arms together. Let $y_{ij}$ represent whether the $j$-th task step of the $i$-th package is a dual-arm action. If it is a dual-arm action, the value is 1, otherwise it is 0. Then the constraint condition is:

% \begin{equation}
%     y_{ij} = 1 \Rightarrow x_{ijk}^L = 1 \land x_{ijk}^R = 1, \forall i,j,k
% \end{equation}

% This ensures that when executing a task step of a dual-arm action, both the left and right arms are in the working state and jointly complete the task.

% \subsubsection{Package Step Merging Constraints}
% \textbf{Package Step Merging Constraints:}Some steps of different packages can be merged. When there are the same operations (such as both requiring using a knife to cut an object), the related objects can be prepared and then the operations can be carried out uniformly. Let $s_{ij}$ represent the operation type of the $j$-th task step of the $i$-th package. If there are different packages $i_1$ and $i_2$, and the operation types of their task steps $j_1$ and $j_2$ are the same (i.e., $s_{i_1j_1} = s_{i_2j_2}$), then these steps can be merged and executed. When planning the task sequence, these steps with the same operation should be preferentially arranged centrally to reduce the time loss caused by operation switching. By introducing specific sorting rules in the optimization process of the objective function, the steps with the same operation can be executed continuously, thus achieving the effect of step merging. 


%%%%%%%%%%
% 需要重新补充公式
\section{Problem Formulation}
\label{sec:Problem_Formulation}

We address the problem of scheduling a set of $m$ tasks, each consisting of $n_i$ sequential operations, on two cooperative robotic arms denoted $L$ and $R$.
%Operations may be executed by a single arm or require both arms simultaneously.
Each operation $o_{ij}$ (the $j$-th operation of task $i$ is either a single-arm operation, executable by either arm, or a dual-arm operation requiring both arms simultaneously.
Our objective is to minimize the makespan $C_{\max}$, defined as the time by which all operations are complete, under grasping, synchronization, and batching constraints:


\begin{equation}
C_{\max} = \max_{i,j} (s_{ij} + p_{ij})
\end{equation}
where \( s_{ij} \) is the start time and \( p_{ij} \) is the processing time of operation \( o_{ij} \).

\begin{itemize}
\item \emph{Grasping Constraint}: At any time instant, each arm can manipulate at most one object. Moreover, once an arm grasps an object, it must continue with operations on that object (or release it) before switching to another.

\item \emph{Dual‐Arm Synchronization Constraint}: For operations requiring both manipulators, the start times must coincide and both arms remain busy while the operation is being jointly executed.

\item \emph{Operation Batching Constraint}: Identical operations (for example, performing operations on different objects using the same tool) across different tasks may be co-scheduled to amortize setup/teardown costs.
\end{itemize}
